Majorana Excitations, Spin- and Mass Currents on the Surface of Topological Superfluid $^3$He-B

The B-phase of superfluid $^3$He is a 3D time-reversal invariant (TRI) topological superfluid with an isotropic energy gap separating the ground-state and bulk continuum states. We report calculations of surface spectrum, spin- and mass current densities originating from the Andreev surface states for confined $^3$He-B. The surface states are Majorana Fermions with their spins polarized transverse to their direction of propagation along the surface. The negative energy states give rise to a ground-state helical spin current confined on the surface. The spectral functions reveal the subtle role of the spin-polarized surface states in relation to the ground-state spin current. By contrast, these states do not contribute to the $T=0$ mass current. Superfluid flow through a channel of confined $^3$He-B is characterized by the flow field, $p_s$. The flow field breaks 2D rotational symmetry and time reversal (T). However, the Bogoliubov-Nambu Hamiltonian remains invariant under $T$ combined with a 180 degree rotation about the normal to the film. As a result the B-phase in the presence of a superflow remains a topological phase with a gapless spectrum of Majorana modes on the surface. Thermal excitation of the Doppler shifted Majorana branches leads to a power law suppression of the superfluid mass current, providing a direct signature of the Majorana branches of surface excitations in the fully gapped 3D topological superfluid, $^3$He-B. Results are reported for the superfluid fraction (mass current) and helical spin current for confined $^3$He-B, including the temperature dependences, as well as dependences on confinement, interactions between quasiparticles and pressure.

==> references-aps.tex <==
% \bibliographystyle{plain}
% \bibliographystyle{apsrev}
% \bibliography{QFS,CM,Books}

\begin{thebibliography}{45}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\expandafter\ifx\csname bibnamefont\endcsname\relax
  \def\bibnamefont#1{#1}\fi
\expandafter\ifx\csname bibfnamefont\endcsname\relax
  \def\bibfnamefont#1{#1}\fi
\expandafter\ifx\csname citenamefont\endcsname\relax
  \def\citenamefont#1{#1}\fi
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem[{\citenamefont{Balatsky et~al.}(2006)\citenamefont{Balatsky, Vekhter,
  and Zhu}}]{bal06}
\bibinfo{author}{\bibfnamefont{A.~V.} \bibnamefont{Balatsky}},
  \bibinfo{author}{\bibfnamefont{I.}~\bibnamefont{Vekhter}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.-X.} \bibnamefont{Zhu}},
  \bibinfo{journal}{Rev. Mod. Phys.} \textbf{\bibinfo{volume}{78}},
  \bibinfo{pages}{373} (\bibinfo{year}{2006}).

\bibitem[{\citenamefont{Sauls and Eschrig}(2009)}]{sau09}
\bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Eschrig}},
  \bibinfo{journal}{New J. Phys.} \textbf{\bibinfo{volume}{11}},
  \bibinfo{pages}{075008} (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Salomaa and Volovik}(1988)}]{sal88}
\bibinfo{author}{\bibfnamefont{M.~M.} \bibnamefont{Salomaa}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{G.~E.} \bibnamefont{Volovik}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{37}},
  \bibinfo{pages}{9298} (\bibinfo{year}{1988}).

\bibitem[{\citenamefont{Vollhardt and W\"olfle}(1990)}]{vollhardt90}
\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Vollhardt}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{W\"olfle}},
  \emph{\bibinfo{title}{{The Superfluid Phases of $^3$He}}}
  (\bibinfo{publisher}{Taylor \& Francis}, \bibinfo{address}{New York},
  \bibinfo{year}{1990}).

\bibitem[{\citenamefont{Qi et~al.}(2009)\citenamefont{Qi, Hughes, Raghu, and
  Zhang}}]{qi09}
\bibinfo{author}{\bibfnamefont{X.-L.} \bibnamefont{Qi}},
  \bibinfo{author}{\bibfnamefont{T.~L.} \bibnamefont{Hughes}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Raghu}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{S.-C.} \bibnamefont{Zhang}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{102}},
  \bibinfo{pages}{187001} (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Volovik}(2009{\natexlab{a}})}]{vol09}
\bibinfo{author}{\bibfnamefont{G.~E.} \bibnamefont{Volovik}},
  \bibinfo{journal}{JETP Lett.} \textbf{\bibinfo{volume}{90}},
  \bibinfo{pages}{587} (\bibinfo{year}{2009}{\natexlab{a}}).

\bibitem[{\citenamefont{Qi and Zhang}(2011)}]{qi11}
\bibinfo{author}{\bibfnamefont{X.-L.} \bibnamefont{Qi}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{S.-C.} \bibnamefont{Zhang}},
  \bibinfo{journal}{Rev. Mod. Phys.} \textbf{\bibinfo{volume}{83}},
  \bibinfo{pages}{1057} (\bibinfo{year}{2011}).

\bibitem[{\citenamefont{Volovik}(2009{\natexlab{b}})}]{vol09a}
\bibinfo{author}{\bibfnamefont{G.~E.} \bibnamefont{Volovik}},
  \bibinfo{journal}{JETP Lett} \textbf{\bibinfo{volume}{90}},
  \bibinfo{pages}{398} (\bibinfo{year}{2009}{\natexlab{b}}).

\bibitem[{\citenamefont{Ryu et~al.}(2010)\citenamefont{Ryu, Schnyder, Furusaki,
  and Ludwig}}]{ryu10}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Ryu}},
  \bibinfo{author}{\bibfnamefont{A.~P.} \bibnamefont{Schnyder}},
  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Furusaki}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{A.~W.~W.} \bibnamefont{Ludwig}},
  \bibinfo{journal}{New Journal of Physics} \textbf{\bibinfo{volume}{12}},
  \bibinfo{pages}{065010} (\bibinfo{year}{2010}).

\bibitem[{\citenamefont{Buchholtz and Zwicknagl}(1981)}]{buc81}
\bibinfo{author}{\bibfnamefont{L.~J.} \bibnamefont{Buchholtz}}
  \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Zwicknagl}},
  \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{B23}},
  \bibinfo{pages}{5788} (\bibinfo{year}{1981}).

\bibitem[{\citenamefont{Hu}(1994)}]{hu94}
\bibinfo{author}{\bibfnamefont{C.~R.} \bibnamefont{Hu}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{72}},
  \bibinfo{pages}{1526} (\bibinfo{year}{1994}).

\bibitem[{\citenamefont{Buchholtz et~al.}(1995)\citenamefont{Buchholtz,
  Palumbo, Rainer, and Sauls}}]{buc95a}
\bibinfo{author}{\bibfnamefont{L.}~\bibnamefont{Buchholtz}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Palumbo}},
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{J. Low Temp. Phys.} \textbf{\bibinfo{volume}{101}},
  \bibinfo{pages}{1079} (\bibinfo{year}{1995}).

\bibitem[{\citenamefont{Matsumoto and Shiba}(1995)}]{mat95}
\bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Matsumoto}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Shiba}}, \bibinfo{journal}{J.
  Phys. Soc. Jpn.} \textbf{\bibinfo{volume}{64}}, \bibinfo{pages}{1703}
  (\bibinfo{year}{1995}).

\bibitem[{\citenamefont{Covington et~al.}(1997)\citenamefont{Covington, Aprili,
  Paraoanu, Greene, Xu, J.Zhu, and Mirkin}}]{cov97}
\bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Covington}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Aprili}},
  \bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Paraoanu}},
  \bibinfo{author}{\bibfnamefont{L.~H.} \bibnamefont{Greene}},
  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Xu}},
  \bibinfo{author}{\bibnamefont{J.Zhu}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{C.~A.} \bibnamefont{Mirkin}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{79}},
  \bibinfo{pages}{277} (\bibinfo{year}{1997}).

\bibitem[{\citenamefont{Fogelstr\"om et~al.}(1997)\citenamefont{Fogelstr\"om,
  Rainer, and Sauls}}]{fog97}
\bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Fogelstr\"om}},
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{79}},
  \bibinfo{pages}{281} (\bibinfo{year}{1997}).

\bibitem[{\citenamefont{Aoki et~al.}(2005)\citenamefont{Aoki, Wada, Saitoh,
  Nomura, Okuda, Nagato, Yamamoto, Higashitani, and Nagai}}]{aok05}
\bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Aoki}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Wada}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Saitoh}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Nomura}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Okuda}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Nagato}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Yamamoto}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Higashitani}},
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Nagai}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{95}},
  \bibinfo{pages}{075301} (\bibinfo{year}{2005}).

\bibitem[{\citenamefont{Choi et~al.}(2006)\citenamefont{Choi, Davis, Pollanen,
  and Halperin}}]{cho06}
\bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Choi}},
  \bibinfo{author}{\bibfnamefont{J.~P.} \bibnamefont{Davis}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Pollanen}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{W.~P.} \bibnamefont{Halperin}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{96}},
  \bibinfo{pages}{125301} (\bibinfo{year}{2006}).

\bibitem[{\citenamefont{Nagato et~al.}(1998)\citenamefont{Nagato, Yamamoto, and
  Nagai}}]{nag98}
\bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Nagato}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Yamamoto}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Nagai}}, \bibinfo{journal}{J.
  Low Temp. Phys.} \textbf{\bibinfo{volume}{110}}, \bibinfo{pages}{1135}
  (\bibinfo{year}{1998}).

\bibitem[{\citenamefont{Vorontsov and Sauls}(2003)}]{vor03}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Vorontsov}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{68}},
  \bibinfo{pages}{064508:1} (\bibinfo{year}{2003}).

\bibitem[{\citenamefont{Murakawa et~al.}(2009)\citenamefont{Murakawa, Tamura,
  Wada, Wasai, Saitoh, Aoki, Nomura, Okuda, Nagato, Yamamoto et~al.}}]{mur09}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Murakawa}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Tamura}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Wada}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Wasai}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Saitoh}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Aoki}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Nomura}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Okuda}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Nagato}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Yamamoto}},
  \bibnamefont{et~al.}, \bibinfo{journal}{Physical Review Letters}
  \textbf{\bibinfo{volume}{103}}, \bibinfo{pages}{155301}
  (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Volovik}(2003)}]{volovik03}
\bibinfo{author}{\bibfnamefont{G.~E.} \bibnamefont{Volovik}},
  \emph{\bibinfo{title}{{The Universe in a Helium Droplet}}}
  (\bibinfo{publisher}{Clarendon Press}, \bibinfo{address}{Clarendon, UK},
  \bibinfo{year}{2003}).

\bibitem[{\citenamefont{Chung and Zhang}(2009)}]{chu09}
\bibinfo{author}{\bibfnamefont{S.~B.} \bibnamefont{Chung}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{S.-C.} \bibnamefont{Zhang}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{103}},
  \bibinfo{pages}{235301} (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Nagato et~al.}(2009)\citenamefont{Nagato, Higashitani,
  and Nagai}}]{nag09}
\bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Nagato}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Higashitani}},
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Nagai}},
  \bibinfo{journal}{J Phys Soc Jpn} \textbf{\bibinfo{volume}{78}},
  \bibinfo{pages}{123603} (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Mizushima et~al.}(2012)\citenamefont{Mizushima, Sato, and Machida}}]{miz12a}
\bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Mizushima}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Sato}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Machida}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{109}},
  \bibinfo{pages}{165301} (\bibinfo{year}{2012}).

\bibitem[{\citenamefont{Mizushima}(2012)}]{miz12}
\bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Mizushima}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{86}},
  \bibinfo{pages}{094518} (\bibinfo{year}{2012}).

\bibitem[{\citenamefont{Hsieh et~al.}(2009)\citenamefont{Hsieh, Xia, Wray,
  Qian, Pal, Dil, Osterwalder, Meier, Bihlmayer, Kane et~al.}}]{hsi09}
\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Hsieh}},
  \bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Xia}},
  \bibinfo{author}{\bibfnamefont{L.}~\bibnamefont{Wray}},
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Qian}},
  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Pal}},
  \bibinfo{author}{\bibfnamefont{J.~H.} \bibnamefont{Dil}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Osterwalder}},
  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Meier}},
  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Bihlmayer}},
  \bibinfo{author}{\bibfnamefont{C.~L.} \bibnamefont{Kane}},
  \bibnamefont{et~al.}, \bibinfo{journal}{Science}
  \textbf{\bibinfo{volume}{323}}, \bibinfo{pages}{919} (\bibinfo{year}{2009}).

\bibitem[{\citenamefont{Zhang et~al.}(1987)\citenamefont{Zhang, Kurkij\"arvi,
  and Thuneberg}}]{zha87}
\bibinfo{author}{\bibfnamefont{W.}~\bibnamefont{Zhang}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Kurkij\"arvi}},
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{E.~V.}
  \bibnamefont{Thuneberg}}, \bibinfo{journal}{Phys. Rev. B}
  \textbf{\bibinfo{volume}{36}}, \bibinfo{pages}{1987} (\bibinfo{year}{1987}).

\bibitem[{\citenamefont{Tsutsumi and Machida}(2012)}]{tsu12b}
\bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Tsutsumi}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Machida}},
  \bibinfo{journal}{Journal of the Physical Society of Japan}
  \textbf{\bibinfo{volume}{81}}, \bibinfo{pages}{074607}
  (\bibinfo{year}{2012}).

\bibitem[{\citenamefont{Balian and Werthamer}(1963)}]{bal63}
\bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Balian}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{N.~R.} \bibnamefont{Werthamer}},
  \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{131}},
  \bibinfo{pages}{1553} (\bibinfo{year}{1963}).

\bibitem[{\citenamefont{Moores and Sauls}(1993)}]{moo93}
\bibinfo{author}{\bibfnamefont{G.~F.} \bibnamefont{Moores}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{J. Low Temp. Phys.} \textbf{\bibinfo{volume}{91}},
  \bibinfo{pages}{13} (\bibinfo{year}{1993}).

\bibitem[{\citenamefont{Lee et~al.}(1999)\citenamefont{Lee, Haard, Halperin,
  and Sauls}}]{lee99}
\bibinfo{author}{\bibfnamefont{Y.}~\bibnamefont{Lee}},
  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Haard}},
  \bibinfo{author}{\bibfnamefont{W.}~\bibnamefont{Halperin}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{Nature} \textbf{\bibinfo{volume}{400}},
  \bibinfo{pages}{431} (\bibinfo{year}{1999}).

\bibitem[{\citenamefont{Sauls}(2000)}]{sau00a}
\bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}}, in
  \emph{\bibinfo{booktitle}{Topological Defects and Non-Equilibrium Symmetry
  Breaking Phase Transitions - {\em Lecture Notes for the 1999 Les Houches
  Winter School}}}, edited by
  \bibinfo{editor}{\bibfnamefont{H.}~\bibnamefont{Godfrin}} \bibnamefont{and}
  \bibinfo{editor}{\bibfnamefont{Y.}~\bibnamefont{Bunkov}}
  (\bibinfo{publisher}{Elsievier Science Publishers},
  \bibinfo{address}{Amsterdam}, \bibinfo{year}{2000}), pp.
  \bibinfo{pages}{239--265}.

\bibitem[{\citenamefont{Schnyder et~al.}(2008)\citenamefont{Schnyder, Ryu,
  Furusaki, and Ludwig}}]{sch08}
\bibinfo{author}{\bibfnamefont{A.~P.} \bibnamefont{Schnyder}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Ryu}},
  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Furusaki}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{A.~W.~W.} \bibnamefont{Ludwig}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{78}},
  \bibinfo{pages}{195125} (\bibinfo{year}{2008}).

\bibitem[{\citenamefont{Serene and Rainer}(1983)}]{ser83}
\bibinfo{author}{\bibfnamefont{J.~W.} \bibnamefont{Serene}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}},
  \bibinfo{journal}{Phys. Rep.} \textbf{\bibinfo{volume}{101}},
  \bibinfo{pages}{221} (\bibinfo{year}{1983}).

\bibitem[{\citenamefont{Andreev}(1964)}]{and64}
\bibinfo{author}{\bibfnamefont{A.~F.} \bibnamefont{Andreev}},
  \bibinfo{journal}{Sov. Phys. JETP} \textbf{\bibinfo{volume}{19}},
  \bibinfo{pages}{1228} (\bibinfo{year}{1964}).

\bibitem[{\citenamefont{Eilenberger}(1968)}]{eil68}
\bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Eilenberger}},
  \bibinfo{journal}{Zeit. f. Physik} \textbf{\bibinfo{volume}{214}},
  \bibinfo{pages}{195} (\bibinfo{year}{1968}).

\bibitem[{\citenamefont{Kurkij\"arvi et~al.}(1987)\citenamefont{Kurkij\"arvi,
  Rainer, and Sauls}}]{kur87}
\bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Kurkij\"arvi}},
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{Can. Journ. Phys.} \textbf{\bibinfo{volume}{65}},
  \bibinfo{pages}{1440} (\bibinfo{year}{1987}).

\bibitem[{\citenamefont{Shelankov}(1980)}]{she80}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Shelankov}},
  \bibinfo{journal}{Sov. Phys. JETP} \textbf{\bibinfo{volume}{51}},
  \bibinfo{pages}{1186} (\bibinfo{year}{1980}).

\bibitem[{\citenamefont{Sauls}(2011)}]{sau11}
\bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{84}},
  \bibinfo{pages}{214509} (\bibinfo{year}{2011}).

\bibitem[{\citenamefont{Volovik}(2010)}]{vol10}
\bibinfo{author}{\bibfnamefont{G.~E.} \bibnamefont{Volovik}},
  \bibinfo{journal}{JETP Lett} \textbf{\bibinfo{volume}{91}},
  \bibinfo{pages}{201} (\bibinfo{year}{2010}).

\bibitem[{\citenamefont{Rainer et~al.}(1996)\citenamefont{Rainer, Sauls, and
  Waxman}}]{rai96}
\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}},
  \bibinfo{author}{\bibfnamefont{J.~A.} \bibnamefont{Sauls}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Waxman}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{54}},
  \bibinfo{pages}{10094} (\bibinfo{year}{1996}).

\bibitem[{\citenamefont{Leggett}(1965)}]{leg65}
\bibinfo{author}{\bibfnamefont{A.~J.} \bibnamefont{Leggett}},
  \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{140}},
  \bibinfo{pages}{A1869} (\bibinfo{year}{1965}).

\bibitem[{\citenamefont{Saunders et~al.}(1981)\citenamefont{Saunders, Wildes,
  Parpia, Reppy, and Richardson}}]{sau81e}
\bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Saunders}},
  \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Wildes}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Parpia}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Reppy}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Richardson}},
  \bibinfo{journal}{Physica B+C} \textbf{\bibinfo{volume}{108}},
  \bibinfo{pages}{791 } (\bibinfo{year}{1981}).

\bibitem[{\citenamefont{Leggett}(1975)}]{leg75}
\bibinfo{author}{\bibfnamefont{A.~J.} \bibnamefont{Leggett}},
  \bibinfo{journal}{Rev. Mod. Phys.} \textbf{\bibinfo{volume}{47}},
  \bibinfo{pages}{331} (\bibinfo{year}{1975}).

\bibitem[{\citenamefont{Haard}(2000)}]{har00}
\bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Haard}}, 
\bibinfo{volume}{{http://spindry.phys.northwestern.edu/he3.htm},}
\bibinfo{journal}{{The $^3$He Calculator}} (\bibinfo{year}{2000}.) 


\bibitem[{\citenamefont{Thuneberg et~al.}(1984)\citenamefont{Thuneberg,
  Kurkij\"arvi, and Rainer}}]{thu84}
\bibinfo{author}{\bibfnamefont{E.}~\bibnamefont{Thuneberg}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Kurkij\"arvi}},
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Rainer}},
  \bibinfo{journal}{Phys. Rev. B} \textbf{\bibinfo{volume}{29}},
  \bibinfo{pages}{3913} (\bibinfo{year}{1984}).

\end{thebibliography}


==> references-arXiv.tex <==
%\bibliographystyle{plain}
% \bibliographystyle{apsrev}
%\bibliography{QFS,CM,Books}

\begin{thebibliography}{10}

\bibitem{and64}
A.~F. Andreev.
\newblock {Thermal Conductivity of the Mixed State of Type II Superconductors}.
\newblock {\em Sov. Phys. JETP}, 19:1228, 1964.

\bibitem{aok05}
Y.~Aoki, Y.~Wada, M.~Saitoh, R.~Nomura, Y.~Okuda, Y.~Nagato, M.~Yamamoto,
  S.~Higashitani, and K.~Nagai.
\newblock Observation of surface andreev bound states of superfluid [sup 3]he
  by transverse acoustic impedance measurements.
\newblock {\em Phys. Rev. Lett.}, 95(7):075301, 2005.

\bibitem{bal06}
A.~V Balatsky, I~Vekhter, and Jian-Xin Zhu.
\newblock Impurity-induced states in conventional and unconventional
  superconductors.
\newblock {\em Rev. Mod. Phys.}, 78(2):373--433, 2006.

\bibitem{bal63}
R.~Balian and N.~R. Werthamer.
\newblock Superconductivity with pairs in a relative p-state.
\newblock {\em Phys. Rev.}, 131:1553, 1963.

\bibitem{buc81}
L.~J. Buchholtz and G.~Zwicknagl.
\newblock Identification of p-wave superconductors.
\newblock {\em Phys. Rev.}, B23:5788, 1981.

\bibitem{buc95a}
L.J. Buchholtz, M.~Palumbo, D.~Rainer, and J.~A. Sauls.
\newblock {Thermodynamics of d-wave Superconductors near a Surface}.
\newblock {\em J. Low Temp. Phys.}, 101:1079, 1995.

\bibitem{cho06}
H.~Choi, J.~P. Davis, J.~Pollanen, and W.~P. Halperin.
\newblock Surface specific heat of $^3$he and andreev bound states.
\newblock {\em Phys. Rev. Lett.}, 96(12):125301, 2006.

\bibitem{chu09}
Suk~Bum Chung and Shou-Cheng Zhang.
\newblock {Detecting the Majorana Fermion Surface State of $^3$He-B through
  Spin Relaxation}.
\newblock {\em Phys. Rev. Lett.}, 103:235301, 2009.

\bibitem{cov97}
M.~Covington, M.~Aprili, E.~Paraoanu, L.~H. Greene, F.~Xu, J.Zhu, and C.~A.
  Mirkin.
\newblock {Observation of Surface-Induced Broken Time-Reversal Symmetry in YBCO
  Tunnel Junctions}.
\newblock {\em Phys. Rev. Lett.}, 79:277, 1997.

\bibitem{eil68}
G.~Eilenberger.
\newblock {Transformation of Gorkov's Equation for Type II Superconductors into
  Transport-Like Equations}.
\newblock {\em Zeit. f. Physik}, 214:195, 1968.

\bibitem{fog97}
M.~Fogelstr\"om, D.~Rainer, and J.~A. Sauls.
\newblock {Tunneling into Current-Carring Surface States of High $T_c$
  Superconductors}.
\newblock {\em Phys. Rev. Lett.}, 79:281, 1997.

\bibitem{har00}
T.~Haard.
\newblock {Helium-Three Calculator}.
\newblock {\em {The $^3$He Calculator}}, {Online:
  http://spindry.phys.northwestern.edu/he3.htm}, 2000.

\bibitem{hsi09}
D.~Hsieh, Y.~Xia, L.~Wray, D.~Qian, A.~Pal, J.~H. Dil, J.~Osterwalder,
  F.~Meier, G.~Bihlmayer, C.~L. Kane, Y.~S. Hor, R.~J. Cava, and M.~Z. Hasan.
\newblock {Observation of Unconventional Quantum Spin Textures in Topological
  Insulators}.
\newblock {\em Science}, 323(5916):919--922, 2009.

\bibitem{hu94}
C.~R. Hu.
\newblock Mid gap states near surfaces of d-wave superconductors.
\newblock {\em Phys. Rev. Lett.}, 72:1526, 1994.

\bibitem{kur87}
J.~Kurkij\"arvi, D.~Rainer, and J.~A. Sauls.
\newblock {Superfluid $^3$He and heavy-fermion superconductors near surfaces
  and interfaces}.
\newblock {\em Can. Journ. Phys.}, 65:1440, 1987.

\bibitem{lee99}
Y.~Lee, T.~Haard, W.P. Halperin, and J.~A. Sauls.
\newblock {Discovery of an Acoustic Faraday Effect in Superfluid $^3$He-B}.
\newblock {\em Nature}, 400:431, 1999.

\bibitem{leg65}
A.~J. Leggett.
\newblock {Theory of a Superfluid Fermi Liquid I: General Formalism and Static
  Properties}.
\newblock {\em Phys. Rev.}, 140:A1869, 1965.

\bibitem{leg75}
A.~J. Leggett.
\newblock {Theoretical Description of the New Phases of Liquid $^3$He}.
\newblock {\em Rev. Mod. Phys.}, 47:331--414, 1975.

\bibitem{mat95}
M.~Matsumoto and H.~Shiba.
\newblock Coexistence of different symmetry order parameters near a surface in
  d-wave superconductors.
\newblock {\em J. Phys. Soc. Jpn.}, 64:1703, 1995.

\bibitem{miz12}
Takeshi Mizushima.
\newblock {Superfluid $^3$He in a restricted geometry with a perpendicular
  magnetic field}.
\newblock {\em Phys. Rev. B}, 86:094518, 2012.

\bibitem{miz12a}
Takeshi Mizushima, Masatoshi Sato, and Kazushige Machida.
\newblock {Symmetry Protected Topological Order and Spin Susceptibility in
  Superfluid $^{3}He-B$}.
\newblock {\em Phys. Rev. Lett.}, 109:165301, 2012.

\bibitem{moo93}
G.~F. Moores and J.~A. Sauls.
\newblock Transverse {W}aves in {S}uperfluid {$^3$He-B}.
\newblock {\em J. Low Temp. Phys.}, 91:13, 1993.

\bibitem{mur09}
S~Murakawa, Y~Tamura, Y~Wada, M~Wasai, M~Saitoh, Y~Aoki, R~Nomura, Y~Okuda,
  Y~Nagato, M~Yamamoto, S~Higashitani, and K~Nagai.
\newblock {New Anomaly in the Transverse Acoustic Impedance of Superfluid
  $^3$He-B with a Wall Coated by Several Layers of $^4$He}.
\newblock {\em Physical Review Letters}, 103(15):155301, 2009.

\bibitem{nag09}
Yasushi Nagato, Seiji Higashitani, and Katsuhiko Nagai.
\newblock {Strong Anisotropy in Spin Suceptibility of Superfluid $^3$He-B Film
  Caused by Surface Bound States}.
\newblock {\em J Phys Soc Jpn}, 78(12):123603, 2009.

\bibitem{nag98}
Yasushi Nagato, Mikio Yamamoto, and Katsuhiko Nagai.
\newblock {Rough Surface Effects on the p-Wave Fermi Superfluids}.
\newblock {\em J. Low Temp. Phys.}, 110(5-6):1135--1171, 1998.

\bibitem{qi09}
Xiao-Liang Qi, Taylor~L. Hughes, S.~Raghu, and Shou-Cheng Zhang.
\newblock {Time-Reversal-Invariant Topological Superconductors and Superfluids
  in Two and Three Dimensions}.
\newblock {\em Phys. Rev. Lett.}, 102(18):187001, 2009.

\bibitem{qi11}
Xiao-Liang Qi and Shou-Cheng Zhang.
\newblock Topological insulators and superconductors.
\newblock {\em Rev. Mod. Phys.}, 83:1057--1110, 2011.

\bibitem{rai96}
D.~Rainer, J.~A. Sauls, and D.~Waxman.
\newblock Current carried by bound states of a superconducting vortex.
\newblock {\em Phys. Rev. B}, 54(14):10094--10106, 1996.

\bibitem{ryu10}
Shinsei Ryu, Andreas~P Schnyder, Akira Furusaki, and Andreas W~W Ludwig.
\newblock Topological insulators and superconductors: tenfold way and
  dimensional hierarchy.
\newblock {\em New Journal of Physics}, 12(6):065010, 2010.

\bibitem{sal88}
M.~M. Salomaa and G.~E. Volovik.
\newblock {Cosmiclike domain walls in superfluid \Heb: Instantons and
  diabolical points in (k,r) space}.
\newblock {\em Phys. Rev. B}, 37:9298--9311, 1988.

\bibitem{sau00a}
J.~A. Sauls.
\newblock {Broken Symmetry and Non-Equilibrium Superfluid $^3$He}.
\newblock In H.~Godfrin and Y.~Bunkov, editors, {\em Topological Defects and
  Non-Equilibrium Symmetry Breaking Phase Transitions - {\em Lecture Notes for
  the 1999 Les Houches Winter School}}, pages 239--265. Elsievier Science
  Publishers, Amsterdam, 2000.

\bibitem{sau11}
J.~A. Sauls.
\newblock {Surface states, Edge Currents, and the Angular Momentum of Chiral
  $p$-wave Superfluids}.
\newblock {\em Phys. Rev. B}, 84:214509, 2011.

\bibitem{sau09}
J.~A Sauls and M~Eschrig.
\newblock {Vortices in Chiral, Spin-Triplet Superconductors and Superfluids}.
\newblock {\em New J. Phys.}, 11:075008, 2009.

\bibitem{sau81e}
J.~Saunders, D.G. Wildes, J.~Parpia, J.D. Reppy, and R.C. Richardson.
\newblock {The normal fraction density in superfluid \Heb}.
\newblock {\em Physica B+C}, 108:791 -- 792, 1981.

\bibitem{sch08}
Andreas~P Schnyder, Shinsei Ryu, Akira Furusaki, and Andreas W.~W Ludwig.
\newblock Classification of topological insulators and superconductors in three
  spatial dimensions.
\newblock {\em Phys. Rev. B}, 78(19):195125, 2008.

\bibitem{ser83}
J.~W. Serene and D.~Rainer.
\newblock {The Quasiclassical Approach to $^3He$}.
\newblock {\em Phys. Rep.}, 101:221, 1983.

\bibitem{she80}
A.L. Shelankov.
\newblock Dragging of normal component by the condensate in nonequimbrium
  superconductors.
\newblock {\em Sov. Phys. JETP}, 51:1186, 1980.

\bibitem{thu84}
E.~Thuneberg, J.~Kurkij\"arvi, and D.~Rainer.
\newblock {Elementary-flux-pinning potential in type-II superconductors}.
\newblock {\em Phys. Rev. B}, 29:3913, 1984.

\bibitem{tsu12b}
Yasumasa Tsutsumi and Kazushige Machida.
\newblock {Edge Current due to Majorana Fermions in Superfluid $^{3}$He A- and
  B-Phases}.
\newblock {\em Journal of the Physical Society of Japan}, 81(7):074607, 2012.

\bibitem{vollhardt90}
D.~Vollhardt and P.~W\"olfle.
\newblock {\em {The Superfluid Phases of $^3$He}}.
\newblock Taylor \& Francis, New York, 1990.

\bibitem{volovik03}
G.~E. Volovik.
\newblock {\em {The Universe in a Helium Droplet}}.
\newblock Clarendon Press, Clarendon, UK, 2003.

\bibitem{vol09a}
G.~E Volovik.
\newblock {Fermion zero modes at the boundary of superfluid $^3$He-B}.
\newblock {\em JETP Lett}, 90:398--401, 2009.

\bibitem{vol09}
G.~E Volovik.
\newblock {Topological Invariant for Superfluid $^3$He-B and Quantum Phase
  Transitions}.
\newblock {\em JETP Lett.}, 90:587--591, 2009.

\bibitem{vol10}
G.~E Volovik.
\newblock {Topological Superfluid \Heb\ in Magnetic Field and Ising Variable}.
\newblock {\em JETP Lett}, 91:201--205, 2010.

\bibitem{vor03}
A.~Vorontsov and J.~A. Sauls.
\newblock {Thermodynamic Properties of Thin Films of Superfluid $^3$He-A}.
\newblock {\em Phys. Rev. B}, 68:064508:1--13, 2003.

\bibitem{zha87}
W.~Zhang, J.~Kurkij\"arvi, and E.~V. Thuneberg.
\newblock {Order parameter of superfluid $^{3}$He-B near surfaces}.
\newblock {\em Phys. Rev. B}, 36:1987--1995, 1987.

\end{thebibliography}

